A Viscous and Heat Conducting Ghost Fluid Method for Multi-Fluid Simulations

The ghost fluid method allows a propagating interface to remain sharp during a numerical simulation. The solution of the Riemann problem at the interface provides proper information to determine interfacial fluxes as well as the velocity of the phase boundary. Then considering two-material problems, the initial states of the Riemann problem belong to different fluids, which may have different equations of states. In the inviscid case, the solution of the multi-fluid Riemann problem is an extension of the classical Riemann problem for a single fluid. The jump of the initial states between different fluids generates waves in both fluids and induces a movement of the interface, similar to a contact discontinuity. More subtle is the extension to viscous and heat conduction terms which is the main focus of this paper. We account for the discontinuous coefficients of viscosity and heat conduction at the multi-fluid interface and derive solutions of the Riemann problem for these parabolic terms, from which we can derive parabolic, interfacial fluxes.

==> packages.tex <==
\RequirePackage{etex}
\usepackage{etoolbox}  %

\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amscd}
\usepackage{amsfonts}
\usepackage{breqn}
\usepackage{mathtools}
\usepackage{nicefrac}
\usepackage[llbracket,rrbracket]{stmaryrd}
\usepackage[normalem]{ulem}

\usepackage{xcolor}

\definecolor{myblue}{RGB}{68,119,170}
\definecolor{mycyan}{RGB}{102,204,238}
\definecolor{mygreen}{RGB}{34,136,51}
\definecolor{myyellow}{RGB}{204,187,68}
\definecolor{myred}{RGB}{238,102,119}
\definecolor{mypurple}{RGB}{170,51,119}
\definecolor{mygrey}{RGB}{187,187,187}


\usepackage{tabularx}
\usepackage{multirow}
\usepackage{multicol}
\usepackage{booktabs} %

\usepackage[format=hang,labelfont=bf]{caption}  %
\usepackage{subcaption}

\usepackage{siunitx}
\sisetup{exponent-product = \cdot, output-product = \cdot}
\sisetup{allow-number-unit-breaks}

\DeclareSIUnit{\angstrom}{\mbox{\normalfont\AA}}
\makeatletter
\DeclareRobustCommand{\AA}{%
  \leavevmode
  \vbox{\ialign{##\cr
    \hidewidth\char'27 \hidewidth\cr
    \noalign{\nointerlineskip\kern-1.4ex}
    A\cr
  }}%
}
\makeatother


\usepackage[capitalise]{cleveref}

\usepackage{changebar}
\usepackage[mode=image]{standalone}
\usepackage{csquotes}  %
\usepackage{xspace}    %

\usepackage[all]{nowidow} %

\frenchspacing %



\usepackage[colorinlistoftodos,prependcaption]{todonotes}
\presetkeys{todonotes}{inline,color=blue!30,size=\footnotesize}{}

\usepackage{morewrites} %

\usetikzlibrary{external}
\tikzexternalize[prefix=tikzfigures/] %

